VAR-DRAM: Variation-Aware Framework for Efficient Dynamic Random Access Memory Design

Dynamic Random Access Memory (DRAM) is the de-facto choice for main memory devices due to its cost-effectiveness. It offers a larger capacity and higher bandwidth compared to SRAM but is slower than the latter. With each passing generation, DRAMs are becoming denser. One of its side-effects is the deviation of nominal parameters: process, voltage, and temperature. DRAMs are often considered as the bottleneck of the system as it trades off performance with capacity. With such inherent limitations, further deviation from nominal specifications is undesired. In this paper, we investigate the impact of variations in conventional DRAM devices on the aspects of performance, reliability, and energy requirements. Based on this study, we model a variation-aware framework, called VAR-DRAM, targeted for modern-day DRAM devices. It provides enhanced power management by taking variations into account. VAR-DRAM ensures faster execution of programs as it internally remaps data from variation affected cells to normal cells and also ensures data preservation. On extensive experimentation, we find that VAR-DRAM achieves peak energy savings of up to 48.8% with an average of 29.54% on DDR4 memories while improving the access latency of the DRAM compared to a variation affected device by 7.4%.

==> Text/ack.tex <==
\section*{Acknowledgment}
\label{sec:ack}
    We would like to thank xyz for his/her contribution in this work. This work is supported grants numbered 1, 2 and 3. Lastly, we would also like to thank anonymous reviewers for their opinions. 


==> Text/dummy-x.tex <==
       \begin{table}[ht]
				\caption{Summary of Proposed and Existing Works}
            \centering
			\begin{tabular}{|p{0.2cm} | p{1.2cm} |p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{1cm}|}
			\hline
          		\multirow{2}{*}{\textbf{Sl.}} & \multirow{2}{*}{\textbf{Name}} & \multirow{2}{*}{\textbf{Savings}} & \multicolumn{3}{|p{2cm}|}{\textbf{Overheads}} & \multirow{2}{*}{\textbf{State}}\\ \cline{4-6}
          		&  & & Perf. & Area & Power &\\ \hline \hline

          		%1. & TAP-low~\cite{liu2010} & 19.90\% &	7.70\% & - & - & Not Preserved \\
                \hline
                1. & Rank Aware~\cite{lu2016} & 24\% &	4\% & 0.40\% & 1.40\% & Cached\\
                \hline
                2. &	PRA~\cite{lee2017}	& 23\% & - & 3\% of a 2Gb DRAM & 0.017\% & Not Applicable\\
                \hline
                %4. &	BAMM~\cite{10.1109} & 6.30\% & 0.70\% & - & - & Not Preserved\\
                %\hline
                3. & RAIDR~\cite{raidr} & 20\% & - & 0.013 mm$^2$ & - & N/A\\
                \hline
                4. &	SPBR~\cite{isqed} & 9.11\% & 0.82\% & $<$1\% of the die & 1.09\%& Preserved\\
                \hline
                5. & Compiler Directed~\cite{delaluz-bank} & 23\% & - & - & - & N/A \\
                %\hline
                %7. & Voltron~\cite{reduced_volt} & 10.5\% & - & - & - & N/A \\
                \hline
                6. & VAR-DRAM & 29.54\% & 0.8\%  & 0.002\%& 1.09\%& Preserved\\
                \hline
                \hline
			\end{tabular}
			\label{tab:summary}
		\end{table} 
		
		
        \begin{figure*}[h]
            \begin{center}
            \mbox{
            \hspace{-1.0ex}
            \subfigure[Energy Savings Across Different Energy Saving Mechanisms]
                {
                \label{fig:energy_comp}
                \includegraphics[width=0.48\textwidth]{Figuresv2/comp_cx.png}
                %\caption{Number of Refresh Instructions Issued}
                }
            \hspace{-1.0ex}
            \subfigure[Bandwidth Case Study for \textit{bwaves}]
                {
                \label{fig:case_bwaves}
                \includegraphics[width=0.48\textwidth]{Figuresv2/scatter.png}
                
                }
            }
            %\vspace{-2.0ex}
            \caption{Comparative Analysis (left) and Bandwidth Analysis (right)}
            %\vspace{-3.0ex}
            \label{fig:ref_all} 
            \end{center}
        \end{figure*}      

==> Text/dummy.tex <==
 \subsection{DRAM Power Components}
    \label{subsec:dram-powp}
        \begin{figure*}[tb]
        \begin{center}
            \mbox{ 
            \hspace{-1.0ex}
            \subfigure[VARIUS~\cite{sarangi} generated map for $L_{eff}$]
                {
                \label{fig:leff_map}
                \includegraphics[width=0.275\textwidth]{power/Figures/leff_var_colored.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[VARIUS~\cite{sarangi} generated map for Capacitance Variance]
                {
                \label{fig:cap_map}
                \includegraphics[width=0.275\textwidth]{power/Figures/cap_var_colored.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Diagram of a 2 Bit Node Trie]
                {
                \label{trie-diag}
                \includegraphics[width=0.325\textwidth]{power/Figures/trie.pdf}
                }
            }
            \vspace{-2.0ex}
            \caption{Distribution Maps (left) and Trie Diagram (right)}
            \vspace{-5.0ex}
            \label{fig:variusanddennsity} 
        \end{center}
    \end{figure*}
    
        \begin{figure*}[tb]
        \begin{center}
            \mbox{ 
            \hspace{-1.0ex}
            \subfigure[Number of Banks Closed = 8]
                {
                \label{fig:8b}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/8.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 16]
                {
                \label{fig:16b}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/16.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 24]
                {
                \label{fig:24b}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/24.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 32]
                {
                \label{fig:32b}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/32.pdf}
                }
            }
%            \caption{Savings observed on closing different banks.}
            \vspace{-6.0ex}
%            \label{fig:result} 
        \end{center}
    \end{figure*}
        \begin{figure*}[tb]
        \begin{center}
            \mbox{ 
            \hspace{-1.0ex}
            \subfigure[Number of Banks Closed = 40]
                {
                \label{fig:40b}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/40.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 48]
                {
                \label{fig:48b}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/48.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 56]
                {
                \label{fig:56b}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/56.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 64]
                {
                \label{fig:64b}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/64.pdf}
                }
            }
            \vspace{-2.0ex}
            \caption{Savings observed on closing different banks.}
%            \vspace{-6.0ex}
            \label{fig:result} 
        \end{center}
    \end{figure*}
    
    \vspace{-3ex}
            \begin{figure*}[tb]
        \begin{center}
            \mbox{ 
            \hspace{-1.0ex}
            \subfigure[Number of Banks Closed = 8]
                {
                \label{fig:40bo}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/8ov.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 16]
                {
                \label{fig:48bo}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/16ov.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 32]
                {
                \label{fig:56bo}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/32ov.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Number of Banks Closed = 64]
                {
                \label{fig:64bo}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/64ov.pdf}
                }
            }
            \vspace{-2.0ex}
            \caption{Performance Overhead Observed on Closing Different Banks}
            \vspace{-5.0ex}
            \label{fig:overh} 
        \end{center}
    \end{figure*}           
            \begin{figure*}[tb]
        \begin{center}
            \mbox{ 
            \hspace{-1.0ex}
            \subfigure[Average Power and Overhead Increment]
                {
                \label{fig:linear}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/linear.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Latency of a 16 GB Memory]
                {
                \label{fig:lat}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/latency16.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Trie Size]
                {
                \label{overhead}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/trie_size.pdf}
                }
            \hspace{-2.0ex}
            \subfigure[Power Required to Maintain the Trie]
                {
                \label{fig:pow_overhead}
                \includegraphics[width=0.24\textwidth]{power/Figures/DDR4/trie_power.pdf}
                }
            }
            \vspace{-2.0ex}
            \caption{Collective Results including Savings/Overhead, Latency, Trie Size and Trie Power}
            \vspace{-5.0ex}
            \label{fig:all_diag} 
        \end{center}
    \end{figure*}
    
                \begin{algorithm}
			\caption{Address Remapping Scheme}
			\label{alg:migrate}
			\begin{algorithmic}[1]
			\STATE Assert: Class PV is instantiated and is valid
			\STATE Ensure V is valid
			\STATE A flag bit FLAG represents reconfigured banks
			\STATE Set $\tau$ = NULL and $\tau_{new}$ = NULL
				\WHILE {$address$}
				\STATE // Resolves address into its corresponding channel, rank, bank, row and column
				\STATE ch, ra, ba, ro, co = resolve($address$, FLAG)
				\STATE // Check for address collision in parallel. Sends interrupt if ro, co mismatches
				\STATE ro', co' = collision\_check ($\tau$, address)
				\IF {PV.calculateVariation (clock)}
%				    \STATE /* calculateVariation () calculates variation maps in simulations or calculates variation based on sensor data (Sec - \ref{sec:hw_impl_para}) on H/W Implementation */
				    \STATE $[\beta[],T[]]$ = PV.getPVVictimTargetPairs (n)
				    %\STATE T = getPVTarget ()
				    \STATE $\tau$ = MigrateAndRemap($\tau$, $\beta$[], T[])
					\IF {$\tau$ != NULL}
						\STATE Power down $\beta$
					\ELSE
						\STATE Continue without migrating
					\ENDIF
				\ENDIF
				\ENDWHILE
			\end{algorithmic}
		    \end{algorithm}
		    
		    %motivation
		     Based on the questions that have been already answered in previous works, we ask four fundamental questions:
    %\begin{enumerate}
    
        \hspace{-0.6cm}    1. Since these variation affected cells are under-performing meaning it has less retention time, lower reliability and higher access latency, is it possible to commensurate the power usage with the quantity of the output it produces?
        
        \hspace{-0.6cm}    2. Instead of using a proportion based model, can we completely power off these cells and devise a mechanism to preserve the data?
        
        \hspace{-0.6cm}    3. What would be the overhead of such a mechanism? Will it marginalize the gains that will be obtained?
    %\end{enumerate}
    
    Our problem hence identified, is implemented and experimented on existing DRAM devices. %We mainly observe the effect of access latency on both healthy and affected devices via \textit{variation aware simulations}. 
    

==> Text/extension.tex <==
\section{Extensions}
\label{sec:extensions}


==> Text/related.tex <==
\section{Related Works}
	\label{sec:related}
	%removed huang, reduced_volt
    Exploring power savings in DRAM devices is one of the key techniques employed in power-efficient systems. Studies such as~\cite{ware, hoelze} reports that DRAM devices consume a significant portion of system's power. 
    %A study by Huang et al.~\cite{huang} reports that DRAM devices consume up to 52\% of the total power. 
    A significant number of prior works have proposed towards saving power for DRAM devices. Delaluz et al.~\cite{delaluz} exploited the prolonged behavior of idle ranks for saving power. Lebeck et al.~\cite{lebeck} demonstrated how a DRAM rank can be transitioned into low power mode. They proposed a method to cluster DRAM accesses into some specific chips so that idle chips can be transitioned into low power mode. This concept of powering down ranks was then established as a standard technique to save power from DRAM devices. Other techniques based on schedulers were then studied in works including~\cite{lebeck,delaluz,delaluz-kande}. The authors in~\cite{delaluz-kande} proposed a method to dynamically map addresses into some specific set of banks in order to exploit power savings. %Cheng et al.~\cite{reduced_volt} proposed a power-saving technique for DRAM devices via voltage scaling. 
    Hassan et al.~\cite{crow} proposed an In-DRAM cache for DRAM based memory systems. The proposed model makes a copy of a DRAM row on the cache. Later, during the execution of the program, if the same row is referenced, it is activated simultaneously from both the primary array, and, as well as from the In-DRAM cache (also known as CROW-cache). Another aspect of saving power in DRAM devices is centered around periodic DRAM refreshes. In the work~\cite{raidr}, the authors propose a selective refresh on variation affected cells in order to maintain the data properly and eliminate unnecessary refreshes. 
	
    Shutting down DRAM banks or transitioning DRAM banks into low power mode is a topic with limited study. Prior works on this aspect include~\cite{delaluz-bank,isqed}, wherein the former, authors propose both software and hardware-based techniques to exploit power savings from DRAM banks. The later attempts to close under-utilized DRAM banks in order to save power. Another work~\cite{bank-sensitive-model} includes a bank sensitive power model for a DRAM power simulator called DRAMPower~\cite{drampower}. The existing implementation of a DRAM module is biased towards power management in a rank wise manner~\cite{micro,ddr4}. Low power memory technologies like LPDDR DRAM have a provision of a bank-wise refresh instead of an all-bank refresh~\cite{microLPDDRx}. The DRAM simulator called DRAMSim2~\cite{dramsim} also implements a heuristics-based technique to demonstrate low power mode in DRAM systems during simulations. Micron Technologies implements a low power mode for idle ranks for their DDR3 DRAM system~\cite{micro} where no I/O accesses are allowed to the rank which results in lower consumption of power. 

    The fabrication process of manufacturing chips is susceptible to variations~\cite{process,sarangi}. These variations lead to the aberration of nominal parameters of P, V, T of these chips. Variation is a well-studied topic for DRAM devices. Hamamoto et al. investigated DRAM data retention distribution in their work~\cite{o34}. They reported that boron concentration in p-well of memory cells characterizes the data retention distribution. Further, variation affects the reliability of the data present on the device which plays an important role in real-time systems and secured systems where corrupt data can lead to catastrophic consequences. Emerging memories and non-volatile memory technologies are gaining momentum in development as these provide a feasible alternative to DRAM-based memories~\cite{nvm}. However, these technologies also have variations~\cite{stt-pv}. Even in flash storage devices like SSD are affected by PV~\cite{other_paper}. 

	Access latency of a DRAM device is affected by PV~\cite{sarangi, process,ras_timing}. Zhao et al.~\cite{process} studied the effects of PV on a DRAM-based last level cache (LLC) where they tried to mitigate slow memory accesses by migrating the data to some other locations of the LLC so that the access latency is maintained uniformly. Sarangi et al.~\cite{sarangi} proposed a statistical method called \textit{VARIUS}, where the decaying portions of a chip can be identified. A study by Ghose et al.~\cite{vampire} concludes that most off-the-shelf DRAM devices are prone to variation. The authors did a study on each granularity of the DRAM device and compared with state-of-the-art simulator results and concluded that there exists a large difference between real and simulated hardware results. Current DDRx DRAM systems perform row migrations in order to mitigate the issue of PV affected defective rows~\cite{sample}. Although this mechanism does mitigate the issue of reliability and access latency, power efficiency, however, is not explored.
	 
	%removed 
	Works have also been done towards preserving the data present in the chips so as to not incur an additional re-computation cost. Prior works on saving the state of the data on caches are done in~\cite{leecho,ozturk,wang}. In~\cite{wang}, the authors propose a technique to design a reliable SNUCA cache for an NoC based CMP. The authors first demonstrate how the chip will degrade over time and subsequently remapped the data without any loss. Lee et al.~\cite{leecho} proposed a bandwidth aware page migration technique for heterogeneous memories.


		
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Sl. No.}} & \multirow{2}{*}{\textbf{Name}} & \multirow{2}{*}{\textbf{Savings}} & \multicolumn{3}{l|}{\hspace{2cm} \textbf{Overhead}}                                   & \multirow{2}{*}{\textbf{State}} \\ \cline{4-6}
   &                   &         & \textbf{Performance} & \textbf{Area}                        & \textbf{Power}   &           \\ \hline \hline
1. & Rank Aware~\cite{lu2016}        & 24\%    & 4\%   & 0.4\%                       & 1.40\%  & Cached    \\ \hline
2. & PRA~\cite{lee2017}               & 23\%    & -     & 3\% of a 2 Gb DRAM          & 0.017\% & N/A       \\ \hline
3. & RAIDR~\cite{raidr}             & 20\%    & -     & 0.013 mm\textsuperscript{2} & -       & N/A       \\ \hline
4. & SPBR~\cite{isqed}                  & 9.11\%                   & 0.82\% & \textless 1\% of 400mm\textsuperscript{2} die & 1.09\% & Preserved              \\ \hline
5. & Compiler Directed~\cite{delaluz-bank} & 23\%    & -     & -                           & -         & N/A       \\ \hline
6. & Voltron~\cite{reduced_volt}           &  10.5\%       & -       &  -                           &  -       & N/A       \\ \hline
7. & BAMM~\cite{10.1109}           &   6.30\%      &  0.70\%     &  -                           & -        & N/A       \\ \hline
8. & TAP-low~\cite{liu2010} & 19.90\% &	7.70\% & - & - & N/A \\ \hline
9. & VAR-DRAM          & 29.54\% & 0.8\% & 0.002\%                     & 1.09\%  & Preserved \\ \hline \hline
\end{tabular}%
}
			\caption{Summary of Proposed and Existing Works}
			\label{tab:summary}
\end{table}		

	To regulate the supply voltage on a device, researchers widely use the concept of power gating~\cite{pg}. This reduces the leakage current of the chip %, especially in unused portions of SRAM technologies. 
	which makes power gated SRAM circuits for implementing sleep mode, which is considered an efficient power management technique. In~\cite{srampg}, the authors propose a \textit{quasi-power-gating} approach in order to reduce leakage power dissipation on SRAM banks. Other applications of power gating are observed in NoCs~\cite{noc1} and Non-Volatile (NV) memory technologies~\cite{nvpg} where the authors proposed a power gated 1 Mb NV embedded memory to optimize the trade-off between macro size and its operational power.

    Hence we conclude that exploitation of DRAM power savings at the bank level is non-existent which is due to the fundamental design of DRAM. Power gating is a technique that has found significant use in NoC architectures but has been sparingly explored in the context of DRAM. PV affected chips normally hinder normal functioning in a real scenario and provides opportunities for optimization. Additionally, data preservation while power-saving leads to significant overheads which may become difficult to mitigate. In Table~\ref{tab:summary}, we show a few DRAM power savings techniques in contrast to each other. %where we can see that the method proposed by us shows the maximal power gain along with data preservation.
